Efficient Reactive Synthesis

Our main result is a polynomial time algorithm for deciding realizability for the GXU sublogic of linear temporal logic. This logic is particularly suitable for the specification of embedded control systems, and it is more expressive than GR(1). Reactive control programs for GXU specifications are represented as Mealy machines, which are extended by the monitoring of input events. Now, realizability for GXU specifications is shown to be equivalent to solving a certain subclass of 2QBF satisfiability problems. These logical problems can be solved in cubic time in the size of GXU specifications. For unrealizable GXU specifications, stronger environment assumptions are mined from failed consistency checks based on Padoa's characterization of definability and Craig interpolation.

==> algorithm.tex <==
\begin{algorithm}
\caption{\textproc{AssumptionRefinement}}
\begin{algorithmic}[1]
\Require{initial specification in GXW: $\phi^{\mathcal{E}} \rightarrow \phi^{\mathcal{S}}$}
\Ensure{conjunction of assumptions $\mathcal{C}^{ref} $ s.t. $\psi \in \mathcal{C}^{ref}$, $\phi^{\mathcal{E}} \wedge \psi \rightarrow \phi^{\mathcal{S}}$ is realizable}
   % \State $\mathcal{C}^{ASS}=\emptyset, \mathcal{V}=\emptyset$ \Comment{$\mathcal{C}^{S}$ is a set of candidate assumptions and $\mathcal{V}$ is a set of assumptions that are visited}
    
    \State $\pi_c=$ \textproc{GetCounterExample($\phi^{\mathcal{E}}\rightarrow \phi^{S}$)}

    \If{$\pi_c= None$}
        \State Return $\{true\}$  \Comment{the given specification is realizable.}

           \EndIf
         
   \State $\mathcal{C}^{ASS}$= \textproc{ComputeInterpolants($\phi^{\mathcal{E}}\rightarrow \phi^{\mathcal{S}}, \pi_c$)} \Comment{$\mathcal{C}^{ASS}$ is a set of assumptions.}
   
   \ForAll{$\phi \in \mathcal{C}^{ASS}$}
    \ForAll{$\phi' \in$ \textproc{AssumptionRefinement($\phi^{\mathcal{E}} \wedge \phi \rightarrow \phi^{\mathcal{S}}$)}}
    \State $\mathcal{C}^{ref}.add(\phi \wedge \phi' )$
    \EndFor
   \EndFor
   
   \State \textbf{return} $\mathcal{C}^{ref}$
   \end{algorithmic}
\end{algorithm}

The GXW specification  is first encoded as SMT formula for realizability checking. If it is unrealizable, a counterexample $\pi$ with assignments of variables is computed. Based on $\pi$, formulae are selected as cores over the variables of $\pi$. The assumptions are too weak because of the missing prediction of variables. 

\begin{algorithm}
\begin{algorithmic}[1]

\caption{ComputeInterpolants}
\Procedure{ComputeInterpolants}{$\phi^{\mathcal{E}} \rightarrow \phi^{\mathcal{S}},\pi $}, \textbf{returns:} assumptions eliminating the counterexample $\pi$
\State $\varphi_{\pi}^{\mathcal{E}}$=\textproc{ SMTEncoding$(\phi^\mathcal{E},\pi)$} , $\varphi_{\pi}^{\mathcal{S}}$=\textproc{ SMTEncoding$(\phi^\mathcal{S},\pi)$}
\State $\mathcal{I}=\textproc{Interpolate}(\varphi_{\pi}^{\mathcal{E}} \wedge \varphi_{\pi}^{\mathcal{S}})$
\If{$\mathcal{I}$==false } 
\State \textbf{return} \{false\}
\Else
\State $\mathcal{F}=\textproc{SMT2GXW}(\mathcal{I})$
\If{$\mathcal{F}$==$\emptyset$ } 
\State \textbf{return} \{false\}
\Else
\State \textbf{return} \textproc{disjuncts($\neg \mathcal{F}$)}
\EndIf
\EndIf
\EndProcedure
\label{interpolants}
\end{algorithmic}
\end{algorithm}

Procedure \textproc{ComputeInterpolants} shown in Algorithm \ref{interpolants} computes an interpolant and translates it to GXW formula to get assumptions. 

==> gxu_synthesis.tex <==
\section{Problem Statement}
Given a \emph{GXU} specification $\varphi(X; Y)$ with input variables $X$ and output variables $Y$, which are assumed to be interpreted over a finite domain $D$, 
we consider the problem of constructing a synchronous program $P_s:  X^+ \to Y$, 
represented as a Mealy machine, such that $P_s$ realizes $\varphi(X; Y)$\@. 
Moreover, if $\varphi(X; Y)$ is unrealizable, our algorithm analyzes the root cause of this unrealizability, and it tries to construct a strengthening of the environment assumption for making at least this strengthened specification realizable. 

Our construction proceeds in two subsequent steps.
    \begin{enumerate}
        \item We first construct a Mealy machine for each of the conjoined \emph{GXU} formulas in a \emph{GXU} specification. 
        \item Conjunctions of individual \emph{GXU} pattern formulas may specify 
              jointly inconsistent behavior.  We therefore define a consistency check for ruling out conjunctions of mutually inconsistent specifications. 
    \end{enumerate}
The first step is a straightforward adaptation of the syntactic translation in~\cite{CYR16} of \emph{GXW} specification formulas into a synchronous program. 
The main difference is in the translation of strong until in \emph{GXU} and the use of Mealy machines with monitoring instead of synchronous dataflow as in~\cite{CLR17,CYR16}\@. 
For details of this syntactic translation we refer the attentive reader to the Appendix~\ref{app:???}\@.

Based on the results of the syntactic transformation of individual formulas into Mealy machines, realizability checking is reduced to checking whether there is any conflict within the Mealy machines. 
These Mealy machines are encoded as QBF formulae. 
 The output of the transitions of Mealy machines, in particular, is expressed by a function vector 
 $\Psi=\langle \psi_1(X),\cdots,\psi_m(X) \rangle$ such that $Y_i \leftrightarrow \psi_i(X)$ and $\exists Y F(X,Y)\equiv F(X,\Psi)$\@. 
 We refer to $\Psi$ as the Skolem function vector and $\psi_i$ as the Skolem function for $Y_i$ that can be considered as an implementation of the controller. 
 Altogether, we construct a QBF $\Phi$ which is satisfiable if and only if the \emph{GXU} 
 specification $\varphi(X; Y)$ is realizable.
 In this way, we are reducing realizability to checking a satisfiability problem.

==> introduction.tex <==
Dependency quantified Boolean formula (DQBF) is a propositional formula extended with universal and existential quantification over propositions extending QBF by henkin quantifiers $\exists x:Y \varphi$ which bind a variable $x$ and specify a dependency set $Y$ of universal variable that $x$ depends on.  DQBF enable widely application in reactive synthesis.  
The problem of {\em reactive synthesis}, in particular, involves the construction of an input-output controller 
as a {\em realization} of a given specification in {\em linear temporal logic} (LTL) over input and output sequences (without further constraining the set of possible inputs)\@. 

Different from QBFs where an existential variable implicityl depends on all the universal variables preceding its quantification level, DQBF specifies the dependency sets explicitly. In order to get unsat cores when the given formula is not satisfiable, we need to dependency elimination and universal reduction by clausal abstraction. We borrow a typical example of DQBF as follows:
\begin{example}
A DQBF $\Psi_1:= \forall x_1 \forall x_2, \exists y_1(x_1) \exists y_2(x_2): x_1 \wedge x_2 \leftrightarrow y_1=y_2$ and a QBF  $\Psi_2:= \forall x_1 \forall x_2, \exists y_1 \exists y_2: x_1 \wedge x_2 \leftrightarrow y_1=y_2$. 
\end{example}
$\Psi_1$ is unsatisfiable while $\Psi_2$ is satisfiable. In formula $\Psi_2$, existential varaibles $y_1$ and $y_2$ both depends on the universal variables $x_1$ and $x_2$. It is obvious that the formula is true when $x_1$ and $x_2$ are true.  


Correct-by-construction program synthesis mechanically translates a problem-specific specification
to a machine-interpretable program that is known to meet the specification~\cite{church1963application}. 
The problem of {\em reactive synthesis}, in particular, involves the construction of an input-output controller 
as a {\em realization} of a given specification in {\em linear temporal logic} (LTL) over input and output sequences (without further constraining the set of possible inputs)\@. 
Solutions to reactive synthesis have been relying on the logic-automaton connection\cite{BL69,Rab72}, and realizability with respect to LTL is 2EXPTIME-complete \cite{RP89,Ros90}\@. 
Despite a long line of impressive research, however, the old dream of correct-by-construction controller synthesis has not made a wide and substantial impact so far on the everyday design of control algorithms. 
As a consequence, embedded control software predominantly still is being developed in low-level, machine-oriented languages -  including ladder diagrams in process automation and sequential programs such as Matlab/Simulink -  which is not only error-prone but also time- and resource-intensive.

Our starting point is the sublogic GXW of LTL as introduced in \cite{CYR16} for the specification of embedded controllers\@.
Informally, GXW includes specifications for input assumptions, invariance conditions on outputs, transition-like reactions of the form $G(in \,\Rightarrow\, X^i out)$, and, more generally, $G(in \,\Rightarrow\, X^i (out\, W \,rel))$, 
where $in$ is a formula whose validity is determined by the next $i$ input valuations\@. 
Hereby, the temporal operator $G$ is the usual universal path quantifier, $X^i$ abbreviates $i$ consecutive next-steps, and $W$ denotes the {\em weak until} temporal operator, the contraint $out$ contains no temporal operators, and the formula $rel$ may contain a fixed number of consecutive next-steps but no other temporal operators for specifying release events. 
The latter reaction formula may consequently be phrased as follows: if there is an input satisfying the constraint $in$ then the $out$ constraint is required to hold on outputs of the controller until there is a $release$ event (or $out$ always holds)\@. 
For these syntactic restrictions of LTL to the temporal operators $G$, $X$, and $W$ we simply refer to this sublogic as GXW\@. 

Despite being rather restrictive, GXW has proven to be expressive enough for specifying typical embedded control scenarios. In particular, we have successfully modeled a large number of  different embedded control scenarios from the industrial automation domain in GXW~\cite{CVR16}\@. 
In addition, GXW has also been used as a formal semantics of the EARS \cite{Mav19} requirements templates for specifying embedded control software in the aerospace industry~\cite{LRSCA17}\@.\footnote{
The EARS template $(while~a, ~when~b~the~system~shall~c~until~d)$, for instance, corresponds to the temporal formula $G(c ~\Rightarrow~(b~W~(d \,\vee\, \neg a))$\@.}

The syntactic restrictions on GXW, on the other hand, allow for a PSPACE synthesis algorithm~\cite{CYR16}\@. 
This algorithm considerably differs from previous approaches for reactive synthesis 
as it generates synchronous dataflow (SDF)~\cite{LM87} instead of gate-level implementations\@.
The GXW synthesis algorithm itself is implemented as part of  {\em autocode4}~\cite{CLR17}\@.
This synthesis tool enables translations of the generated SDFs to control languages such as SCADE/Lustre, and it maintains an explicit traceability relation, as required by current safety certification regimes, between the GXW controller specifications and the generated SDF implementations.
Experimental results with {\em autocode}, as reported in~\cite{CYR16}, suggest that GXW synthesis scales well to industrial-sized control problems\@.
Consequently, synthesis tools such as {\em autocode4} may seamlessly be integrated into industrial tool chains for developing mission- and safety-critical embedded control systems. 

Specification, however, is arguably the most important and also the most challenging design step for embedded control, and specifications often are too weak, too strong, vacuous, or not realizable.
Based on an understanding of the intended control and the inner workings of the intended operating environment, a human engineer may still be able to capture the intended behavior of embedded controllers in the face of inadequate specifications.
Automated synthesis algorithms, however, lack these human-like interpretative skills, and therefore they need to rely on adequate specifications for correctly and completely capturing intended control behaviors for all possible environment behaviors

We therefore are developing a procedure for supporting the development of realizable control specifications by means of constructing suitable constraints on the possible behaviors of the environment. 
Consider, for example, the specification $G(in \Rightarrow X out) ~\land~G(out \Rightarrow X \neg out)$~\cite{CHJ08}\@. 
The specification is not realizable because whenever $in$ holds in two consecutive steps, the 
system cannot produce a value for $out$ such that this specification is satisfied.
Therefore, we need to constrain the possible behavior of the environment to make it realizable.
A possible candidate is $G(in \Rightarrow X \neg in)$\@. 
Further candidates such as $false$ are unsatisfactory, since they make the specification trivially realizable.
In general there are several possible restrictions on the environment, but not all of them are satisfactory. 
The challenge of assumption mining is to find environment restrictions that is sufficient, does not restrict system behavior, and still gives the environment maximal freedom~\cite{CHJ08}\@.  

Solutions to assumption mining  have previously been studied for different variations of the problem of reactive synthesis~\cite{CHJ08,alur2015pattern,cavezza2017interpolation,cavezza2020minimal,alrajeh2020adapting}\@.
They all rely on repairing unrealizable specifications by means of constructing witness traces which can not be controlled by the system and restricting the set of possible environment behaviors accordingly. 

In contrast to previous approaches, which are based on complex determinization operations and non-emptiness checks for $\omega$-automata, we are developing a procedure for assumption mining which is solely based on logical operations. This has several advantages as we can build on established theorem proving capabilities such as {\em minimal unsatisfiable cores} for explaining and pinpointing at the underlying reason of unrealizability, and the construction of {\em interpolation} formulas for restricting environment behavior.
In order to keep the presentation of our assumption mining algorithm as simple as possible, we restrict ourselves, in the tradition of reactive synthesis, to the synthesis of finite-state systems. 
However, extensions to timed specifications and specifications modulo useful theories such as linear and non-linear arithmetic are straightforward as long as the underlying logics are decidable and we can construct minimal unsatisfiable cores and interpolation formulas.

Our assumption mining procedure involves the following three consecutive steps.
   \begin{itemize}
       \item For a given GXW specification $\phi^E \Rightarrow \phi^S$ we construct a 2QBF formula $\Psi$ such that $\Psi$ is satisfiable if and only if $\phi^E \Rightarrow \phi^S$ is realizable; this construction basically follows the GXW synthesis algorithm in~\cite{CYR16}\@.
       \item If $\neg\Psi$ is satisfiable, we obtain a counterstrategy from a satisfying witness, and we    ... unsat core ...
       \item .... interpolation to eliminate counterstrategies to make the specification realizable. 
   \end{itemize}
   
 The paper is structured as follows. 
 In Section~\ref{???} we describe a simple railway interlocking system, which is used throughout this paper as running example and for illustrating the individual steps of our assumption mining algorithm for GXW.
 Section~\ref{???} briefly reviews necessary background material on GXW and actor-based reactive synthesis as the basis for constructing a 2QBF formula from a GXW specification, which is satisfiable if and only if the GXW specification is realizable. 
 Then, in Section~\ref{???} ...
 Section~\ref{???} includes an in-depth comparison with related work on assumption mining for reactive systems, and we conclude with some final remarks in Section~\ref{???}\@.


==> introduction2.tex <==
% \section{Introduction}
Solutions to {\em reactive synthesis} 
for generating machine-interpretable controllers 
from task-specific input-output specifications
have traditionally been relying on the logic-automaton
connection~\cite{buchi1990solving,rabin1969decidability}.
Despite a long line of impressive technical 
results~\cite{pnueli1989synthesis,bohy2012acacia+,filiot2011antichains,jobstmann2006optimizations,faymonville2017encodings,finkbeiner2012lazy,jobstmann2007anzu,schewe2007bounded,kupferman2005safraless,schewe2007bounded},
however, reactive synthesis has not actually succeeded in making a 
deep impression on the way we are designing control programs. 
As a consequence, embedded control software  still is predominantly being developed in rather low-level machine-oriented programming languages, such as ladder diagrams in process automation, which is not only error-prone but also time- and resource-intensive.

A major cause for this theory-practice gap
is a certain lack of formal specifications in industrial design flows 
of both the control program and its operating context. 
Our starting point in addressing this issue are established semi-formal specification languages for embedded control systems such as EARS~\cite{mavin2009easy} and CLEAR~\cite{hall2018clear,hall2021knowledge}, 
as there usually is a straightforward formal interpretation of specification templates in these languages in terms of a small number of temporal logic patterns~\cite{rolls10227just}\@. 
Consider, for example, the EARS specification template
   \begin{center}
       When $T$ the system shall $A$ until $R$,
   \end{center}
where $T$ is the rule trigger, $A$ is the specification of control actions, and $R$ the release condition. 
These kinds of templates are easily encoded in a fragment of {\em linear temporal logic} (LTL) by
    $$\mathbf{G}\,(T \rightarrow (A \,\mathbf{U}\, R))\mbox{\@,}$$
where $\mathbf{G}$ are the "globally" 
and $\mathbf{U}$ the "strong until" operators of LTL\@.
In addition, these constraints may contain any number of next-step ($\mathbf{X}$) temporal operators. 
In this way, EARS specification templates are expressible in a sublogic of LTL without nested until operators~\cite{LRSCA17}\@.

We simply call the resulting logic GXU, because of the restriction of LTL to the $\mathbf{G}$, $\mathbf{X}$,
and $\mathbf{U}$ temporal operators~\cite{cheng2016structural}\@. 
This logic builds upon GXW~\cite{CYR16,CLR17}, 
which is slightly weaker in that it only supports "weak until" but not "strong until"\@.
This fragment of LTL has proven, despite its severe syntactic restrictions, to be expressive for modeling
a large number of embedded control scenarios from the 
industrial automation domain~\cite{CVR16}\@. 
%The generated data flow programs can be integrated into industrial design flows, for example, by compiling them into industrial design languages such as Scade, LabView, Mathlab/Simulink, and continuous function charts (IEC 61131-3)~\cite{cheng2017autocode4,cheng2014g4ltl}, and they might also be compiled into performant, deterministic, and concurrent systems~\cite{lee1987synchronous,lohstroh2021toward}\@.The generated code may also be used in safety-related applications, since a traceability relation between specification and code is maintained,  as  mandated byapplicable safety engineering practices such as IEC 61508, DO 178C, and ISO 26262\@. 

The specification of the operating context, arguably, is the most challenging design step for embedded control, and these specifications often are too weak, too strong, vacuous, or not realizable.
Based on an understanding of the intended control and the inner workings of the intended operating environment, a human engineer is often able to capture the intended behavior of embedded controllers in the face of inadequate specifications.
Automated synthesis algorithms, however, lack these human-like interpretative skills, and therefore they need to rely on adequate specifications for correctly and completely capturing intended control behaviors for all possible environment behaviors.

We therefore are developing a procedure for supporting the development of realizable control specifications by means of constructing suitable constraints on the possible behaviors of the environment. 
Consider, for example, the GXU specification
     \begin{align}
     \mathbf{G}(in \rightarrow \mathbf{X} out) ~\wedge~
         \mathbf{G}(out \rightarrow \mathbf{X} \neg out)\mbox{\@.} 
      \end{align}
This specification is not realizable because whenever $in$ holds in two consecutive steps, the 
system cannot produce a value for $out$ such that this specification is satisfied.
Therefore, we first need realizability checking and then  to constrain the possible behavior of the environment to make it realizable if it is unrealizable. Solutions to realizability checking have previously been studied for different variations of the problem of reactive synthesis~\cite{CHJ08,alur2015pattern,cavezza2017interpolation,cavezza2020minimal,alrajeh2020adapting,dimitrova2019synthesizing,baumeister2020explainable,li2011mining}\@.
They usually rely on repairing unrealizable specifications by means of constructing witness traces which can not be controlled by the system and restricting the set of possible environment behaviors accordingly. In contrast to previous approaches, which are based on complex determination operations and non-emptiness checks for $\omega$-automata, we are developing a procedure not relying on complicated automaton models and constructions. Instead, we proceeds by recursion on the structure of the control 
specification for constructing mealy machines by predefined pattern, for example, for monitoring inputs events, 
measuring the time steps passed since notable events, and they are generating corresponding control events. Realizability checking can be solved by conflict detection within those mealy machines. Then we use QBF encoding for transition constraints of mealy machines and candidate skolem functions. Thus, realizability checking can be reduced to satisfiability checking for the given candidate skolem functions. The procedure can be decided in polynomial time. Meanwhile, if it is unrealizable, we develop a procedure for assumption mining which is solely based on logical operations via unsat formula obtained by satisfiability checking. This has several advantages as we can build on established concepts from logic such as {\em Padoa's} characterization of definability, {\em  unsatisfiable sub-formula} for explaining and pinpointing at the underlying reason of unrealizability, 
and the construction of {\em interpolation} formulas for restricting environment behavior. As a result, it is able to find environment restrictions that is sufficient, does not restrict system behavior, and still gives the environment maximal freedom~\cite{CHJ08}\@  
%In the previous example, a possible candidate is $\mathbf{G}(in \Rightarrow \mathbf{X} \neg in)$\@. 
%Further candidates such as $\text{false}$ are unsatisfactory, since they make the specification trivially realizable.
%In general there are several possible restrictions on the environment, but not all of them are satisfactory. 
%The challenge of {\em assumption mining} is to find environment restrictions that is sufficient, does not restrict system behavior, and still gives the environment maximal freedom~\cite{CHJ08}\@.  

Our main contributions are as follows.
\begin{itemize}
     \item Definition of the GXU logic, which is strictly more expressive than GXW \cite{CYR16,CLR17} and GR(1) \cite{bloem2012synthesis}\@; 
     \item \textcolor{blue}{ A novel data stream representation named Mealy machine with monitor where each transition is equipped with a nested automaton for monitoring input event once trigger condition holds, the transition produces output event}\@; 
       \item \textcolor{blue}{An polynomial-time synthesis procedure for GXU specifications, which is based on a reduction of the realizability problem to a consistency checking  in a quantified Boolean logic for skolem functions}; 
     \item \textcolor{blue}{A novel method for assumption mining for unrealizable specifications, which is based on logic context including Padoa's theorem, unsatisfiable sub-formula and interpolation rather than complicated automata constructions.} 
\end{itemize}
%In order to keep the presentation of our assumption mining algorithm as simple as possible, we restrict ourselves, in the tradition of reactive synthesis, to the synthesis of finite-state systems. 
%However, extensions to timed specifications and specifications modulo useful theories such as clock constraints and even more arithmetic are straightforward as long as the underlying constraint logic is decidable, and as long as one can construct unsatisfiable cores and interpolation formulas in these logics. 


The paper is structured as follows.
Section 2 review the preliminaries including notations of propositional logic, QBF, LTL and realizability of reactive system.   Next, Section 3 describes the definition of GXU specification. Section 4 discusses the problem we would like to solve in this paper.  The main technical contributions are given in Section 5, which includes how to use mealy machine to present streams satisfying the given GXU formula,  how to check realizability based on QBF encoding and how to generate assumption refinements to make it realizable.
Section 6 illustrates a case study to demonstrate how our approach works in industrial domain.   In Section 7, we discuss our results  with most closely related work on reactive synthesis. 
 We conclude with some final remarks in Section 8.

